Buffer Anytime: Zero-Shot Video Depth and Normal from Image Priors

We present Buffer Anytime, a framework for estimation of depth and normal maps (which we call geometric buffers) from video that eliminates the need for paired video--depth and video--normal training data. Instead of relying on large-scale annotated video datasets, we demonstrate high-quality video buffer estimation by leveraging single-image priors with temporal consistency constraints. Our zero-shot training strategy combines state-of-the-art image estimation models based on optical flow smoothness through a hybrid loss function, implemented via a lightweight temporal attention architecture. Applied to leading image models like Depth Anything V2 and Marigold-E2E-FT, our approach significantly improves temporal consistency while maintaining accuracy. Experiments show that our method not only outperforms image-based approaches but also achieves results comparable to state-of-the-art video models trained on large-scale paired video datasets, despite using no such paired video data.

==> sec/3_method_old.tex <==
\section{Method}
\label{sec:method}

We first formulate our problem as follows: Given a input RGB video consists of $M$ frames, $\bm{I}_{1,...,M} \in \mathbb{R}^{3\times M}$, we aim to predicts the corresponding depth maps $\bm{\mathcal{D}}_{1,...,M}\in \mathbb{R}^M$, and surface normal maps $\bm{\mathcal{N}}_{1,...,M}\in \mathbb{R}^{3\times M}$ represented in the camera coordinates. For convenience, we will mainly focus on describing the task of depth estimation without loss of generality. Existing state-of-the-art methods for video geometry prediction models are commonly trained from sufficient paired datasets, i.e. a set of data pairs $(\bm{I}_{1,...,M}, \bm{\hat{\mathcal{D}}}_{1,...,M})_{1,...,N_{data}}$ of input frames and ground truth depth maps. 
Our model on the other hand, does not require any paired video datasets, instead only relies on video data $(\bm{I}_{1,...,M})_{1,...,N_{data}}$. 

The key insight of our approach is to combine image-based diffusion prior and optical-flow based smooth control. Suppose we have an image depth prediction model $f^{img}_\theta(\bm{I})=\bm{\mathcal{D}}^{img}$ trained by the large-scale image paired datasets to reconstruct the underlying data prior $p^{img}( \bm{\mathcal{D}} | \bm{I})$, our goal is to develop an upgraded video model $f^{vid}_\theta$ that backboned by $f^{img}_\theta$ and able to predict depth maps from videos, i.e.  $f^{vid}_\theta(\bm{I}_{1,...,M})=\bm{\mathcal{D}}^{vid}_{1,...,M}$. The prediction of $f^{vid}_\theta$ should satisfy two conditions: First, each frame of the depth prediction $\bm{\mathcal{D}}^{vid}_i$ should accommodate the image data prior $p^{img}( \bm{\mathcal{D}} | \bm{I})$ and second, the frames of the prediction should be smooth and consistent with each other. 

\subsection{Training Pipeline}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/training.pdf}
  \caption{\textbf{Visualization of Our Training Pipeline}. \fujun{Figure text size too small}}
  \label{fig:pipeline}
\end{figure}

To achieve the goal of our video depth and normal prediction, two losses are applied for the training of our method: the optical flow based smooth loss as described in \ref{sec:of}, and a regularization loss that enforces the model to produces the results aligned with the image model. In depth estimation, the regularization loss is based on the affine-invariant relative loss in Depth Anything~\cite{DepthAnythingV1}: 
\begin{equation}
\mathcal{L}_{depth} = \frac{1}{|\bm{\mathcal{D}}_i|}||\bm{\hat\mathcal{D}}'_i - \bm{\mathcal{D}}'_i||_2,
\end{equation}
where $\bm{\mathcal{D}}'_i$ is the predicted depth map of the i'th frame normalized by the offset $t=\text{median}(\bm{\mathcal{D}}_i)$ and the scale $s=\frac{1}{|\bm{\mathcal{D}}_i|}\sum_{x} |\bm{\mathcal{D}}_i(x) - t|$, $\bm{\hat\mathcal{D}}'_i$ is the normalized depth map from the image model. 
% In practice, we observe that calculating the regularization loss at a random frame in each iteration is sufficient to let the model keep the image prior. 
In normal estimation, we leverage the latent representation of the backbone model, and simply apply an L2 loss on the predicted latent maps $\bm{z}$:
\begin{equation}
\mathcal{L}_{normal} = \frac{1}{|\bm{z}_i|}||\bm{\hat z }_i - \bm{z}_i||_2.
\end{equation}
To speedup, we randomly select one frame from the video in each iteration and calculate the regularization loss on this frame only. The overall training loss is:
\begin{equation}
    \mathcal{L} = \omega_{reg}\mathcal{L}_{depth/normal} + \mathcal{L}_{sm}.
\end{equation}
$\omega_{reg}$ is is set to $1$ in all experiments. Fig.~\ref{fig:pipeline} shows the pipeline structure. Aside from the video model, a fixed pre-trained image model and a optical flow model are also deployed in the pipeline. We calculate the single frame prediction and the optical flow maps in a just-in-time manner.
Partically, calculating the smooth loss for the normal model requires decoding the output latent maps into RGB frames first, which is impractical to be applied to all frames at once due to memory limit. Hence we apply the deferred back-propagation technique introduced in~\cite{ARF}. Here, we first split the latent map into chunks of 4 frames, then calculate the smooth loss for each chunk at a time and back-propagating the gradients to the chunks. We concatenate the gradients of all chunks together as the gradient of the whole latent maps. 



\subsection{Optical Flow Based Smoothness Guidance}
\label{sec:of}

\begin{figure}[t]
  \centering
  \includegraphics[width=\linewidth]{figures/opticalflow.pdf}
  \caption{\textbf{Illustration of our masking procedure for the optical flow loss}. }
  \label{fig:of}
\end{figure} 

As Fig.~\ref{fig:concept} shows, image predictors usually suffers from inconsistent results across frames due to the ambiguity of affine transformation (i.e. scale and offset) of the prediction and uncertainty from the model. To alleviate this problem, a reasonable approach is to align the depth predictions between the corresponding pixels across different frames.  
Inspired by NVDS\cite{NVDS}, we apply a pre-trained optical flow estimator to calculate the correspondence between adjacent frames for the smooth loss calculation. Specifically, let say the predicted optical flow maps between two adjacent frames $\bm{I}_k, \bm{I}_{k+1}$ are $\bm{\mathcal{O}}_{k\rightarrow k+1}$ and $\bm{\mathcal{O}}_{k+1\rightarrow k}$, then a simple smooth loss between the two frames can be defined as:

\begin{align}
\mathcal{L}_{sm} &= \frac{1}{|\bm{I_k}|}\sum_{\bm{x}\in \bm{I_k}}|\bm{I}_k(\bm{x}) - \bm{I}_{k+1}(\bm{\mathcal{O}}_{k\rightarrow k+1}(\bm{x}))|_1 \\
&+ \frac{1}{|\bm{I}_{k+1}|}\sum_{\bm{x}}|\bm{I}_{k+1}(x) - \bm{I}_{\bm{x}}(\bm{\mathcal{O}}_{k+1\rightarrow k}(\bm{x}))|_1
\end{align}

In practice, however, the optical flow prediction can be inaccurate or wrong due to the incapacity of the pretrained model, affecting the effectiveness of the loss as Fig.~\ref{fig:of} shows. To prevent that, we add two more filtering methods to curate the correctly corresponded pixels across the frames.
The first method applies the cycle-validation technique that is commonly used in many previous image correspondence methods~\cite{}. Here we only select the pixels in $\bm{I}_k$ that satisfies:
\begin{align}
||\bm{\mathcal{O}}_{k\rightarrow k+1}(\bm{\mathcal{O}}_{k+1\rightarrow k}(\bm{x})) - x||_2 \leq \tau_{c},
\end{align}
where $\tau_{c}$ a hyper-parameter as a threshold. The second technique is based on the observation that the smooth loss can be incorrectly overestimated near the boundary areas in the depth frames due to the inaccuracy of the optical flow. Our solution to this problem is to apply the canny edge detector~\cite{CANNY} on predicted depth maps, and then filter out the losses on the pixels that are close to the detected edges (i.e. the Manhatten distance is smaller than $3$ pixels). The combination of the two filters effectively removes the outliers and improves the robustness of of our model, which we will show in our experiments.


% Several recent works \cite{} show that the task of image-to-buffer generation can be achieved in a single step. Different from traditional diffusion models, the single-step models are only trained with the largest timestep $t=T$. During inference, the model predict the results from a pure gaussian noise within one iteration. These line of works not only provide a more efficient and better solution for the image-to-buffer problem, also bypasses the procedure of blending noises and ground truth as model input in the traditional diffusion model training, shedding lights on our task, video-to-buffer without direct supervision.

\subsection{Model Architecture}

\begin{figure*}[h]
  \centering
  \includegraphics[width=\linewidth, height=0.5\linewidth]{figures/Network.pdf}
  \caption{\textbf{Our Network Architecture}.  }
  \label{fig:architecture}
\end{figure*} 

In order to generate consistent and high-fidelity video results across frames, choosing a robust and stable the image-based backbone model that preserves the structure of the input frames is crucial: it can greatly reduce the inconsistency and ambiguity of the image results, facilitating our video model training process. Thankfully, recent advances in large-scale image-to-depth and image-to-normal models have brought up many powerful candidates. In this work, we opt to use Depth Anything V2~\cite{DepthAnythingV2} for the backbone of our depth prediction model, and Marigold E2E FT~\cite{Marigold E2E FT} for our normal prediction model. 

Depth Anything V2~\cite{DepthAnythingV2} is a Dense Vision Transformer (DPT)~\cite{DPT} that consists of a Vision Transformer (ViT)~\cite{ViT} as an encoder, and a light weighted refinement network that fuse the feature outputs of several ViT blocks together and produces the final results. Here we freeze the ViT backbone and only fine-tune the refinement network. As Fig.~\ref{fig:architecture} (a) shows, we inject three temporal blocks in between the fusion blocks, as a bridge to connect the latent maps across different frames. Notice that the ViT blocks are fully detached from the gradient flow, which helps reducing the memory cost during the training, enabling supports for longer video. 

MariGold-E2E-FT~\cite{MarigoldE2EFT} is a Latent Diffusion Model~\cite{LDM} built upon Stable-Diffusion V2.0~\cite{StableDiffusionV2}. 
% In general, a diffusion model aims to to recover a data distribution $p_0$ from the Gaussian distribution $p_T$ by reversing a diffusion process, the process that starts from a data $x_0$ and gradually adds noise to the data until it become indistinguishable to a Gaussian noise $\epsilon\sim p_T $. 
In general, a Diffusion Model~\cite{DDPM, DDIM, ScoreMatching} aims to generate results from a sampled Gaussian noise $x_T$ by gradually denoising it to the clean data $x_0$. In each step $t\in T,...,1$, it predicts the noise $\epsilon$ added to the input $x_t$ and denoise it to $x_{t-1}$. To train a diffusion model, one should first construct a $x_t$ blended by a data point $x_0$ and a sampled noise $\epsilon$, then ask the model to recover $x_0$ from $x_t$. 
Particularly, MariGold-E2E-FT is designed to work in a special case where the model skips all the intermediate states $x_{T-1}$ to $x_{1}$ and directly predict $x_0$ from pure noise $x_T$. This setting is crucial to our scenario where no ground truth data exists, since it avoids using any data $x_0$ to assemble the model input $x_t$ for training. Here, we opt to apply the common practice in video diffusion model works that inserting temporal layer in-between the spatial layers, as Fig.~\ref{fig:architecture} (b) demonstrates. The original U-Net layers and the Autoencoder are both fixed during the training. % 

The temporal blocks in both model are samely structured as the blocks in AnimateDiff~\cite{AnimateDiff}, which consists of several temporal attention blocks followed by a projection layer. The final projection layer of each block are zero-initialized to ensure the model acting the same as the image model when the training begins.

% To train a diffusion model with a data point $p_0$, one should first blend a data $x_0$ with a sampled noise $\epsilon$ to a noise level $x_t$, than train the model reconstruct the $x_0$ from $x_t$. 
% generate results $x_0$ from gaussian noises $x_T=\epsilon$ through a series of denoising process in timesteps $t\in1,2,...,T$. In each denoising step, a denoising network predicts the $x_0$ from the current state $x_t$. It then samples $x_{t-1}$ from the predicted $x_0$ and $x_t$. To train a diffusion model with ground truth data $x_0$, one should first sample a noise $\epsilon$ from the gaussian distribution, then MariGold-E2E-FT is specially designed to sample from zero maps using only one timestep.

% Here we opt to apply the common practice in video diffusion model training that inserting temporal layer in-between the spatial layers. The original U-Net layers and the AutoEncoder are both fixed during the training. The temporal blocks in both models are samely structured as the blocks in  AnimateDiff~\cite{AnimateDiff}. 


==> sec/4_experiments_old.tex <==

\section{Experiment}

\begin{table*}[t]
\centering

\caption{\textbf{Evaluation on the video depth estimation.} The methods in the first chunk are video methods trained on video dataset, and methods in the second chunk are image models. We also report the average inference time of each method (normalized by its frame size compared to ours) on the KITTI dataset. *Some methods performs slightly different from what reported in DepthCrafter in our tests. }
\label{tab:depth}

{\small \begin{tabular}{lc ccc c ccc c ccc}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Time } & \multicolumn{3}{c}{ScanNet}  && \multicolumn{3}{c}{KITTI}  &&  \multicolumn{3}{c}{Bonn} \\ %& Rank.\\
\cline{3-5} \cline{7-9} \cline{11-13} 
& & AbsRel $\downarrow$  & $\delta_1$ $\uparrow$ & OPW $\downarrow$ && AbsRel $\downarrow$ & $\delta_1$$\uparrow$ & OPW $\downarrow$ && AbsRel $\downarrow$  & $\delta_1$ $\uparrow$ & OPW $\downarrow$  \\
\midrule

ChronoDepth~\citep{ChronoDepth} & 106s &
0.159  & 0.783 & 0.040 &&
0.151$^*$  & 0.797$^*$ & 0.023 && 
0.109$^*$  & 0.886$^*$ & 0.024 \\

NVDS~\citep{NVDS} & 283s &
0.187  & 0.677 & 0.062 &&
0.253  & 0.588 & 0.045 && 
0.210$^*$  & 0.693$^*$ & 0.047 \\

DepthCrafter~\citep{DepthCrafter} & 270s &
\rsecond{0.125}  & \rsecond{0.848} & \rsecond{0.036} &&
\rfirst{0.110}  & \rfirst{0.881} & 0.049 && 
\rfirst{0.075}  & \rfirst{0.971} & \rsecond{0.020} \\

\midrule

MariGold~\citep{MariGold} & 475s &
0.166  & 0.769 & 0.108 &&
0.149  & 0.796 & 0.110 && 
0.091  & \rsecond{0.931} & 0.077  \\

% LOTUS~\citep{LOTUS} &&
%  &  & &&
%  &  &  && 
%  &  &  \\

% Geowizard~\citep{Geowizard} &
%   &  & &&
%   &  &  && 
%   & &  \\

% Geowizard-E2E-FT~\citep{E2EFT} &&
%   &  &  &&
%   &  &  && 
%   &  &  \\

MariGold-E2E-FT~\citep{E2EFT} & 72s &
0.150  & 0.802 & 0.063 &&
0.151  & 0.779 & 0.049 && 
\rsecond{0.090}  & 0.921 & 0.037 \\

DA V2~\citep{DepthAnythingV2} & 31s &
0.135  & 0.822 & 0.055 &&
0.140  & 0.804 & \rsecond{0.041} && 
0.118$^*$  & 0.875$^*$ & 0.041 \\

\bottomrule
Ours (DA V2) & 33s &
\rfirst{0.123}  & \rfirst{0.853} & \rfirst{0.034} &&
\rsecond{0.119}  & \rsecond{0.865} & \rfirst{0.018} && 
0.102  & 0.925 & \rfirst{0.019} \\
\end{tabular}}

\end{table*}

\begin{table*}[t]
\centering

\caption{\textbf{Evaluation on the video normal estimation.}}
\label{tab:normal}

{\small \begin{tabular}{l cccc c cccc }
\toprule
\multirow{2}{*}{Method} & \multicolumn{4}{c}{Sintel}  && \multicolumn{4}{c}{ScanNet} \\
\cline{2-5} \cline{7-10}
& Mean $\downarrow$ & Median $\downarrow$ & $11.25^\circ$ $\uparrow$ & OPW $\downarrow$ && Mean $\downarrow$ & Median $\downarrow$  &  $11.25^\circ$ $\uparrow$ & OPW $\downarrow$   \\
\midrule

DSINE~\citep{DSINE} &
35.710  & 29.707 & 51.700 & 0.039 &&
22.754 & 11.438 & 77.564 & 0.070 \\

Marigold ~\citep{MariGold} &
& & & &&
& & &  \\

% Geowizard ~\citep{Marigold} &
% & & & &&
% & & &  \\

Marigold-E2E-FT ~\citep{E2EFT} &
32.858 & 27.300 & 55.289 & 0.052 &&
21.587 & 9.951 & 78.547 & 0.052 \\

Ours (Marigold-E2E-FT) &
33.421 & 28.320 & 54.188 & 0.018 &&
21.263 & 9.976 & 79.060 & 0.040 \\

\end{tabular}}


\end{table*}


\begin{table}[t]
\centering

\caption{\textbf{Ablation Study on KITTI depth estimation.}}
\label{tab:normal}

{\small \begin{tabular}{l ccc}
\toprule
Method & AbsRel $\downarrow$  & $\delta_1$ $\uparrow$ & OPW $\downarrow$  \\
\midrule
Ours $w_{reg}=0.1$ & 
0.137 & 0.846 & 0.018 \\
Ours $w_{reg}=3$ & 
0.122 & 0.860 & 0.019 \\
Ours no mask & 
0.122 & 0.860 & 0.017 \\
Ours all frames & 
 0.120 & \rfirst{0.865} & \rfirst{0.017} \\
Ours & 
 \rfirst{0.119} & \rfirst{0.865} & 0.018 \\

\end{tabular}}

\end{table}


\subsection{Implementation Details}
All of our model are built with the PyTorch~\cite{Pytorch} library. We use the official implementation of Depth Anything V2~\cite{Depth Anything V2} and Marigold-E2E-FT~\cite{MarigoldE2EFT}, and the temporal blocks are adopted from the implementation of the AnimateDiff in Diffusers~\cite{Diffusers}. All of our experiments are conducted on NVIDIA H100 GPUs with 80GB memory, and based on the memory budget, we opt to set the maximum video length to be 110 frames for depth estimation, and 32 frames for normal estimation. 

Our training data consists of about 200K videos collected by ourselves, and each clip contains 128 frames. We use the AdamW~\cite{AdamW} optimizer for both experiments, and the learning rate is set to $10^{-4}$ for depth and $10^{-5}$ for normal. A warm-up process with $1000$ timesteps is applied at the beginning of the training, linearly increasing the learning rate from $0$ to the set value. The training runs on $24$ H100 GPUs with the total batch size of $24$. We also apply the Exponential-Moving-Averaging~\cite{EMA} techniques in the training with the decay coefficient set to $0.999$. The training takes approximately 1 day for $20,000$ iterations. 


\subsection{Video Depth Estimation Results}
We use the benchmark provided by the state-of-the-art video depth model DepthCrafter~\cite{DepthCrafter} to quantitatively compare our method and the baselines. This benchmark is modified from the commonly used image depth evaluation~\cite{DepthAnythingV2, MariGold, Geowizard} for testing video depth models. Specifically, for each test video, we first solve a global affine transformation (a offset and a scale) shared by all frames that best aligns the prediction to the ground truth, than evaluate on the affinity transformed prediction maps. We report three different types of metrics: The Mean Absolute Relative Error (\textit{AbsRel}), the percentage of pixels that has the prediction depth in between $\frac{1}{1.25}$ and $1.25$ times the ground truth depth ($\delta$1), and the optical-flow based smooth error (\textit{OPW}) that is defined in the save way of our smooth loss. Tests are conducted on three different datasets: ScanNet~\cite{ScanNet} is a dataset of static indoor scenes; KITTI~\cite{KITTI} is a street-view dataset with LiDAR depth annotations; and Bonn~\cite{Bonn} is a small scale dynamic indoor dataset. We use the same test data selection as the ones in DepthCrafter.
The results are shown in Tab.~\ref{tab:depth}. Our model brings a huge improvement to the backbone model Depth Anything V2~\cite{DepthAnythingV2} in terms of the output quality and smoothness, and even being comparable to the DepthCrafter, the state-of-the-art model trained video large-scale annotated video datasets, on the ScanNet and KITTI dataset. 

We also demonstrate the qualitative comparisons on Fig.~\ref{fig:depth}, showing the consistency and quality of our model visually. \zhengfei{Add more comment when the image is ready.}




\subsection{Video Normal Estimation Results}
To the best of our knowledge, there is no publicity available benchmark tailored for video normal estimation, hence we opt to set up our own benchmark based on the image model setting from~\cite{DSINE}. We select two datasets from the original benchmark that contains continuous input frames, one is the Sintel~\cite{Sintel} dataset (A synthetic dataset of dynamic scenes) and the other is the ScanNet~\cite{scannet} dataset. Different from the original setting, we evenly sample 32 frames from each data scene as a test video. We report three image-based metrics: the mean and median value of the angle between the predicted and ground truths normals, the percentage of predictions that has angle to the ground truth less than $11.25^\circ$, plus the video smooth metric introduced in the depth evaluation. Results are shown in Tab.~\ref{tab:normal}. For the image-based metrics, our model performs comparably as the image backbone, showing that our model well preserve the prior from the image model. It is also reasonable to see that there is no marginal improvement here, since the advantages a video model can take on these metrics are limited. On the other hand, however, our model has much better performance on the smooth metric, indicating its powerful capability to produce temporal consistent and smooth results. This is also demonstrated in our visual results in Fig.~\ref{fig:normal}.

\subsection{Ablation Study}
To verify our design, we also conduct an ablation study on the depth estimation task on the KITTI dataset. We compare our model with 4 variant: \textit{Ours $\omega_{reg}=0.1$} and  \textit{Ours $\omega_{reg}=3$} are models trained with different weights on the regularization loss; \textit{Ours no mask} is the model trained on the smooth loss without masking out invalid optical flow correspondences; \textit{Ours all frames} is the model trained with all frames for regularization instead of a single frame. Our full model outperforms all of the first three variants, showing the effectiveness of our design and configuration. On the other hand, \textit{Ours all frames} doesn't not achieve better results than the regular model, showing that the regularization loss on single frame is already sufficient to align the model with the image prior.




\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth, height=0.75\linewidth]{figures/holder.png}
  \caption{\textbf{Qualitative comparison on Video Depth Estimation}. }
  \label{fig:depth}
\end{figure*} 

\begin{figure*}[t]
  \centering
  \includegraphics[width=\linewidth,height=0.75\linewidth]{figures/holder.png}
  \caption{\textbf{Qualitative comparison on Video Normal Estimation}. }
  \label{fig:normal}
\end{figure*} 
